K2-288Bb: A Small Temperate Planet in a Low-mass Binary System Discovered by Citizen Scientists

Observations from the Kepler and K2 missions have provided the astronomical community with unprecedented amounts of data to search for transiting exoplanets and other astrophysical phenomena. Here, we present K2-288, a low-mass binary system (M2.0 +/- 1.0; M3.0 +/- 1.0) hosting a small (Rp = 1.9 REarth), temperate (Teq = 226 K) planet observed in K2 Campaign 4. The candidate was first identified by citizen scientists using Exoplanet Explorers hosted on the Zooniverse platform. Follow-up observations and detailed analyses validate the planet and indicate that it likely orbits the secondary star on a 31.39-day period. This orbit places K2-288Bb in or near the habitable zone of its low-mass host star. K2-288Bb resides in a system with a unique architecture, as it orbits at >0.1 au from one component in a moderate separation binary (aproj approximately 55 au), and further follow-up may provide insight into its formation and evolution. Additionally, its estimated size straddles the observed gap in the planet radius distribution. Planets of this size occur less frequently and may be in a transient phase of radius evolution. K2-288 is the third transiting planet system identified by the Exoplanet Explorers program and its discovery exemplifies the value of citizen science in the era of Kepler, K2, and the Transiting Exoplanet Survey Satellite.

==> AO_text.tex <==
\subsection{High-resolution Imaging}\label{subsec:hri}

As part of our standard process for validating transiting exoplanets, we observed EPIC~210693462 with infrared high-resolution adaptive optics (AO) imaging at Keck Observatory.  The Keck Observatory observations were made with the NIRC2 instrument on Keck-II behind the natural guide star AO system.  The observations were made on 2017~Aug~20 in the narrow-band $Br-\gamma$, the H-continuum, and J-continuum filters in the standard 3-point dither pattern that is used with NIRC2 to avoid the left lower quadrant of the detector which is typically noisier than the other three quadrants. The dither pattern step size was $3\arcsec$ and was repeated three times, with each dither offset from the previous dither by $0.5\arcsec$.  The observations utilized an integration time of 6.6, 4.0, and 2.903 seconds, respectively, with one coadd per frame for a total of 59.4, 36, and 3.92 seconds.  The camera was in the narrow-angle mode with a full field of view of $10\arcsec$ and a pixel scale of approximately $0.009942 \arcsec$ per pixel. The Keck AO observations clearly detected a nearly equal brightness companion approximately $0.8\arcsec$ to the southeast of the primary target. 

The NIRC2 AO data have a resolution of 0.049$^{\prime\prime}$ (FWHM) in the $Br$-$\gamma$ filter, 0.040$^{\prime\prime}$ (FWHM) in the $H$-$cont$, and 0.039$^{\prime\prime}$ (FWHM) in the $J$-$cont$ filter. The sensitivities of the AO data were determined by injecting fake sources into the final combined images with separations from the primary targets in integer multiples of the central source's FWHM \citep{furlan2017}.  The sensitivity curves shown in Figure \ref{fig:ao_contrast} represent the 5$\sigma$ limits of the imaging data. The companion separation was measured from the $Br$-$\gamma$ image and found to be $\Delta\alpha = 0.259\arcsec \pm 0.001\arcsec$ and $\Delta\delta = -0.746\arcsec \pm 0.001\arcsec$.  The presence of the blended companion must be taken into account to obtain the correct transit depth and planetary radius \citep{ciardi2015}.

The stars have blended 2MASS magnitudes of $J = 10.545 \pm 0.026$ mag, $H=9.946 \pm 0.020$ mag and $K_s = 9.724 \pm 0.023$ mag.  The stars have measured magnitude differences of $\Delta J = 4.97 \pm 0.04$ mag, $\Delta H = 4.96 \pm 0.03$ mag, and $\Delta K_s = 0.988 \pm 0.003$ mag. $Br$-$\gamma$ has a central wavelength that is sufficiently close to $Ks$ to enable the deblending of the 2MASS magnitudes into the two components.  The primary star has deblended real apparent magnitudes of $J_1 = 10.910 \pm 0.027$ mag, $H_1 = 10.313 \pm 0.021$ mag, and $Ks_1 = 10.0918 \pm 0.023$ mag, corresponding to $(J-H)_1 = 0.597 \pm 0.033$ mag and $(H-K_s)_1 = 0.221 \pm 0.031$ mag. The companion star has deblended real apparent magnitudes of $J_2 = 11.907 \pm 0.0269$ mag, $H = 11.303 \pm 0.021$ mag, and $Ks_2 = 11.079 \pm 0.023$ mag, corresponding to $(J-H)_2 = 0.604 \pm 0.033$ mag and $(H-K_s)_2 = 0.224 \pm 0.031$ mag. Utilizing the $(Kepmag - Ks)\ vs.\ (J-Ks)$ color relationships \citep{howell2012}, we derive approximate deblended Kepler magnitudes of the two components of $Kepmag_1 = 13.46\pm0.09$ mag and $Kepmag_1 = 14.49\pm0.10$ mag, for Kepler magnitude difference of $\Delta Kepmag = 1.03\pm0.12$ mag, which is used when fitting the light curves and deriving a true transit depth.

Both stars have infrared colors that are consistent with an M3V spectral type (Figure~\ref{fig:cc}).  It is unlikely that the star is a heavily reddened background star. Based upon an $R=3.1$ extinction law, an early-K star would have to be attenuated by more than 1 magnitude of extinction to make the star appear as a mid M-dwarf.  The entire line-of-sight extinction through the Galaxy is only $A_V\approx0.7$~mag at this location in the galaxy \citep{sf2011} making a background star an unlikely source of the detected companion. 

References used:

\bibitem[Ciardi et al.(2015)]{ciardi2015} Ciardi, D.~R., Beichman, C.~A., Horch, E.~P., \& Howell, S.~B.\ 2015, \apj, 805, 16 

\bibitem[Furlan et al.(2017)]{furlan2017} Furlan, E., Ciardi, D.~R., Everett, M.~E., et al.\ 2017, \aj, 153, 71

\bibitem[Howell et al.(2012)]{howell2012} Howell, S.~B., Rowe, J.~F., Bryson, S.~T., et al.\ 2012, \apj, 746, 123 

\bibitem[Schlafly \& Finkbeiner(2011)]{sf2011} Schlafly, E.~F., \& Finkbeiner, D.~P.\ 2011, \apj, 737, 103 




